Leveraging Multiple Teachers for Test-Time Adaptation of Language-Guided Classifiers

Recent approaches have explored language-guided classifiers capable of classifying examples from novel tasks when provided with task-specific natural language explanations, instructions or prompts (Sanh et al., 2022; R. Menon et al., 2022). While these classifiers can generalize in zero-shot settings, their task performance often varies substantially between different language explanations in unpredictable ways (Lu et al., 2022; Gonen et al., 2022). Also, current approaches fail to leverage unlabeled examples that may be available in many scenarios. Here, we introduce TALC, a framework that uses data programming to adapt a language-guided classifier for a new task during inference when provided with explanations from multiple teachers and unlabeled test examples. Our results show that TALC consistently outperforms a competitive baseline from prior work by an impressive 9.3% (relative improvement). Further, we demonstrate the robustness of TALC to variations in the quality and quantity of provided explanations, highlighting its potential in scenarios where learning from multiple teachers or a crowd is involved. Our code is available at: https://github.com/WeiKangda/TALC.git.

==> llm_baseline_table.tex <==
\begin{table}[t!]
\footnotesize
\begin{center}
\begin{tabular}{ lrrr} 
 \toprule

\textbf{\textbf{Tasks}} & \begin{tabular}{@{}c@{}}T0\end{tabular} & OPT & \begin{tabular}{@{}c@{}}FLAN-T5\\-XXL\end{tabular}\\
 \midrule
 banknote-authentication & $44.7$ & $44.7$  & $54.2$ \\ 
 tic-tac-toe-endgame & $67.7$ & $32.3$  & $32.3$ \\
 car-evaluation & $3.8$  & $2.3$  & $3.8$ \\
contraceptive-choice & $23.4$ & $27.5$  & $38.3$\\
 indian-liver-patient & $67.8$ & $32.2$ & $66.1$\\
 travel-insurance & $38.9$ & $42.5$ & $71.9$\\
 \midrule
 \textbf{Average} & $41.1$ & $30.2$ & $44.4$ \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-0.1in}
\caption{Results of using different LLMs by prompting the models with all explanations concatenated. Comparing Table~\ref{tab:llm-results} and Table~\ref{tab:llm-baseline-results}, \nalla still outperforms LLMs when using the same LLMs as language-guided classifier.
}
\vspace{-0.1in}
\label{tab:llm-baseline-results}
\end{table}
